A Greedy Approach to Adapting the Trace Parameter for Temporal Difference Learning

One of the main obstacles to broad application of reinforcement learning methods is the parameter sensitivity of our core learning algorithms. In many large-scale applications, online computation and function approximation represent key strategies in scaling up reinforcement learning algorithms. In this setting, we have effective and reasonably well understood algorithms for adapting the learning-rate parameter, online during learning. Such meta-learning approaches can improve robustness of learning and enable specialization to current task, improving learning speed. For temporal-difference learning algorithms which we study here, there is yet another parameter, $\lambda$, that similarly impacts learning speed and stability in practice. Unfortunately, unlike the learning-rate parameter, $\lambda$ parametrizes the objective function that temporal-difference methods optimize. Different choices of $\lambda$ produce different fixed-point solutions, and thus adapting $\lambda$ online and characterizing the optimization is substantially more complex than adapting the learning-rate parameter. There are no meta-learning method for $\lambda$ that can achieve (1) incremental updating, (2) compatibility with function approximation, and (3) maintain stability of learning under both on and off-policy sampling. In this paper we contribute a novel objective function for optimizing $\lambda$ as a function of state rather than time. We derive a new incremental, linear complexity $\lambda$-adaption algorithm that does not require offline batch updating or access to a model of the world, and present a suite of experiments illustrating the practicality of our new algorithm in three different settings. Taken together, our contributions represent a concrete step towards black-box application of temporal-difference learning methods in real world problems.

==> Definitions.tex <==
\RequirePackage{latexsym}
\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{bm}
\RequirePackage{enumitem}


%%%%%%%% Distribution definitions %%%%%%%%%%%%%%%

\newcommand{\normal}{\mathcal{N}}
\newcommand{\Lg}{\mathcal{L}}
\newcommand{\given}{|}

%%%%%%%% Matrix/vector definitions %%%%%%%%%%%%%%%

\newcommand{\inlinevec}[2]{%
  \ensuremath{\Bigl[\negthinspace\begin{smallmatrix}#1\\#2\end{smallmatrix}\Bigr]}}
\newcommand{\inlinemat}[4]{%
  \ensuremath{\Bigl[\negthinspace\begin{smallmatrix}#1 \ \ #2 \\#3 \ \ #4\\\end{smallmatrix}\Bigr]}}
\newcommand{\mathvec}[2]{\left[\begin{array}{c}#1\\#2\end{array} \right] }

\renewcommand{\vec}[1]{\mathbf{\boldsymbol{#1}}}
%\newcommand{\makevector}[1]{{\mathbf #1}}
\newcommand{\zerovec}{\vec{0}}
\newcommand{\onevec}{\vec{1}}
\newcommand{\one}{\mathbf{1}}  % Identity
\newcommand{\zero}{\mathbf{0}} % Zero
\newcommand{\eye}{\mathbf{I}}

%%%%%%%% Simple math functions %%%%%%%%%%%%%%%
\newcommand{\pinv}{\dagger}
\newcommand{\sgrad}{\partial}
\newcommand{\sign}[1]{\mathrm{sign}(#1)}
\newcommand{\posdef}{\succeq}
%\newcommand{\e}{{\textrm{e-}}}
\newcommand{\Dom}{{\textrm{Dom}}}
\newcommand{\smallinv}[1]{{#1}^{\scalebox{0.5}[0.5]{\( - 1\)}}}

%%%%%%%% Norm definitions %%%%%%%%%%%%%%%
\newcommand{\frob}[1]{\left\| #1 \right\|_F}
\newcommand{\frobsq}[1]{\left\| #1 \right\|_F^2}
\newcommand{\frobsqn}[1]{\| #1 \|_F^2}
\newcommand{\frobsqtr}[1]{\text{tr}\left(#1'#1\right)}
\newcommand{\sqnorm}[1]{\left\|  #1 \right\|_{2}}
\newcommand{\spnorm}[1]{\left\|  #1 \right\|_{sp}}
\newcommand{\tracenorm}[1]{\left\|  #1 \right\|_{tr}}
\newcommand{\twonorm}[1]{\left\|  #1 \right\|_2}
\newcommand{\twoone}[1]{\left\|  #1 \right\|_{2,1}}
\newcommand{\bregman}[3]{D_{#1}(#2 \; || \: #3)}

%%%%%%%% Widely accepted Sets and Symbols %%%%%%%%%%%%%%%

\newcommand{\CC}{\mathbb{C}} % Complex numbers
\newcommand{\EE}{\mathbb{E}} % Expectation
\newcommand{\FF}{\mathbb{F}} % Fexpectation
\newcommand{\HH}{\mathbb{H}} % Arbitrary field
\newcommand{\II}{\mathbb{I}} % Delta Indicator
\newcommand{\KK}{\mathbb{K}} % Arbitrary field
\newcommand{\MM}{\mathbb{M}} % Median
\newcommand{\NN}{\mathbb{N}} % Natural numbers
\newcommand{\PP}{\mathbb{P}} % Probability
\newcommand{\QQ}{\mathbb{Q}} % Rationals
\newcommand{\RR}{\mathbb{R}} % RR numbers
\newcommand{\RRbar}{\overline{\RR}} % RR numbers
\newcommand{\VV}{\mathbb{V}} % Variance
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}} % Integers

% Set of [0, infty]
\newcommand{\RRpos}{{\RR^+}}

%%%%%%%% Mathematical Operations %%%%%%%%%%%%%%%

\newcommand*{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand*{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand*{\arginf}{\mathop{\mathrm{arginf}}}
\newcommand*{\argsup}{\mathop{\mathrm{argsup}}}
\newcommand{\bd}{\mathop{\mathrm{bd}}}
\newcommand{\cl}{\mathop{\mathrm{cl}}}
\newcommand{\core}{\mathop{\mathrm{core}}}
\newcommand{\co}{\mathop{\mathrm{co}}}
\newcommand{\col}{\mathop{\mathrm{col}}}
%\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\const}{\mathrm{constant}}
\newcommand{\dom}{\mathop{\mathrm{dom}}}
\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\eigs}{\mathop{\mathrm{eigs}}}
\newcommand{\emp}{\mathop{\mathrm{emp}}}
\newcommand{\intr}{\mathop{\mathrm{int}}}
\newcommand{\nulls}{\mathop{\mathrm{null}}}
\newcommand*{\mini}{\mathop{\mathrm{minimize}}}
\newcommand*{\maxi}{\mathop{\mathrm{maximize}}}
\newcommand{\nnz}{\mathop{\mathrm{nnz}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}}
\newcommand{\ri}{\mathop{\mathrm{ri}}}
\newcommand{\row}{\mathop{\mathrm{row}}}
\newcommand{\sgn}{\mathop{\mathrm{sign}}}
\newcommand{\spec}{\mathop{\mathrm{sp}}}
\newcommand{\sspan}{{\textrm{span}}}
\newcommand{\svd}{\mathop{\mathrm{svd}}}
\newcommand{\te}{\mathop{\mathrm{te}}}
\newcommand{\traj}{\mathop{\mathrm{Traj}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\vect}{\mathop{\mathrm{vec}}}
\DeclareMathOperator\arctanh{arctanh}
%\newcommand{\ln}{\mathop{\mathrm{ln}}}

%%%%%%%% Utility functions %%%%%%%%%%%%%%%

\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\mydet}[1]{\det\left[ #1 \right]}
\newcommand{\myspan}[1]{\mathrm{span}\cbr{#1}}
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}
\newcommand{\pwrt}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ppwrt}[1]{\frac{\partial^2}{(\partial #1)^2}}
\newcommand{\aleq}{\preccurlyeq}
\newcommand{\ageq}{\succcurlyeq}
\newcommand{\set}[2]{\{#1 \ | \ #2\}}
\newcommand{\subfigurespace}[1]{ % Reasonable value = 0.1
\begin{minipage}[b]{#1\textwidth}
 \textbf{ }
 \end{minipage}}
 \newcommand{\figspace}{\begin{minipage}[b]{0.1\textwidth} \textbf{ } \end{minipage}}
\newcommand{\unaryminus}{\scalebox{0.75}[1.0]{\( - \)}}

%%%%%%%% Brackets %%%%%%%%%%%%%%%

\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\ccc}[1]{|\!|\!|#1|\!|\!|}
\newcommand{\sembrack}[1]{[\![#1]\!]}


%%%%%%%% Text definitions %%%%%%%%%%%%%%%

\newcommand{\apriori}{{\emph{a priori}}}
\newcommand{\emphdef}[1]{\textbf{#1}}
\newcommand{\introword}[1]{\textbf{\emph{#1}}}
\newcommand{\emphstart}[1]{\textbf{#1}}
\newcommand{\ea}{\emph{et al.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\iid}{\text{i.i.d.}}
\newcommand{\cf}{\emph{cf.}\ }
\newcommand{\wrt}{\emph{w.r.t.}\ }
\newcommand{\subheader}[1]{
\vspace{8pt}
\noindent
{\large\bfseries #1}}

%%%%%%%% Examples of Stock standard definitions %%%%%%%%%%%%%%%
% This is just here as a reference for naming convention

%\newcommand{\xb}{\mathbf{x}}
%\newcommand{\xbtil}{\tilde{\xb}}
%\newcommand{\xtil}{\tilde{x}}
%\newcommand{\xhat}{\hat{x}}
%\newcommand{\xbhat}{\hat{\xb}}
%\newcommand{\Xtil}{\tilde{X}}
%\newcommand{\xbar}{\bar{x}}
%\newcommand{\xbbar}{\bar{\xb}}
%\newcommand{\Xb}{\mathbf{X}}
%\newcommand{\Xbtil}{\tilde{\Xb}}
%\newcommand{\Xbar}{\bar{X}}
%\newcommand{\Xbbar}{\bar{\Xb}}
%\newcommand{\Xhat}{\hat{X}}
%\newcommand{\Xbhat}{\hat{\Xb}}
%\newcommand{\Xcal}{\mathcal{X}}
%\newcommand{\Xtilde}{\widetilde{X}}
%\newcommand{\xvec}{\vec{x}}
%\newcommand{\Xvec}{\vec{X}}
%\newcommand{\xvecbar}{\bar{\vec{x}}}
%\newcommand{\xvechat}{\hat{\vec{x}}}
%\newcommand{\valhat}{\hat{\val}}

%%%%%%%% Theorems and Friends %%%%%%%%%%%%%%%

%% Some style files might actually define these variables.
%% So don't mess with them if they are already defined

\ifx\BlackBox\undefined
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\fi

\ifx\QED\undefined
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\fi

\newcommand{\eproof}{$\null\hfill\blacksquare$}
%\ifx\proof\undefined
\renewenvironment{proof}{\par\noindent{\bf Proof:\ }}{\eproof} %{\hfill\BlackBox\\[.3mm]}
\newenvironment{proofsketch}{\par\noindent{\bf Proof Sketch:\ }}{\eproof} %{\hfill\BlackBox\\[.3mm]}
%\fi
%\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}

% If end proof with align, then can add a negative space to bring up proof box
\newcommand{\palignbox}{\par \vspace{-0.8cm}}

\newif\ifsamenumbers

\ifx\theorem\undefined
\newtheorem{theorem}{Theorem}
\fi

\ifx\example\undefined
\newtheorem{example}{Example}
\fi

\ifx\property\undefined
\newtheorem{property}{Property}
\fi

\ifx\lemma\undefined
\ifsamenumbers
\newtheorem{lemma}[theorem]{Lemma}
\else
\newtheorem{lemma}{Lemma}
\fi
\fi

\ifx\proposition\undefined
\ifsamenumbers
\newtheorem{proposition}[theorem]{Proposition}
\else
\newtheorem{proposition}{Proposition}
\fi
\fi

\ifx\remark\undefined
\newtheorem{remark}{Remark}
\fi

\ifx\corollary\undefined
\ifsamenumbers
\newtheorem{corollary}[theorem]{Corollary}
\else
\newtheorem{corollary}{Corollary}
\fi
\fi

\ifx\definition\undefined
\newtheorem{definition}{Definition}
\fi

\ifx\conjecture\undefined
\ifsamenumbers
\newtheorem{conjecture}[theorem]{Conjecture}
\else
\newtheorem{conjecture}{Conjecture}
\fi
\fi

\ifx\axiom\undefined
\newtheorem{axiom}{Axiom}
\fi

\ifx\claim\undefined
\ifsamenumbers
\newtheorem{claim}[theorem]{Claim}
\else
\newtheorem{claim}{Claim}
\fi
\fi

\ifx\assumption\undefined
\newtheorem{assumption}{Assumption}
\fi

% \renewcommand{\qedsymbol}{$\blacksquare$}
\newcommand{\myintertext}[1]{\end{enumerate} #1\begin{enumerate}[resume]}
\newenvironment{cenumerate}{%
\vspace{10pt}
\noindent{\Large\bfseries Contributions:}
\begin{enumerate}[label={\textbf{Contribution \arabic*.}\ },leftmargin=0cm,itemindent=.5cm,labelwidth=\itemindent,labelsep=0cm,align=left]
}
{\end{enumerate}}

%%%%%%%% Various Optimizers %%%%%%%%%%%%%%%

\newcommand{\BMRM}{{\sf BMRM}}
\newcommand{\bmrm}{{\sf BMRM}}
\newcommand{\cpm}{{\sf CPM}}
\newcommand{\liblinear}{{\sf liblinear}}
\newcommand{\lsbmrm}{{\sf ls-bmrm}}
\newcommand{\qpbmrm}{{\sf qp-bmrm}}
\newcommand{\pegasos}{{\sf pegasos}}
\newcommand{\pegan}{{\sf pegasos-$n$}}
\newcommand{\pegaone}{{\sf pegasos-1}}
\newcommand{\svmstruct}{{\sf SVM-Struct}}
\newcommand{\svmperf}{{\sf SVM-Perf}}
\newcommand{\nest}{{\sf pragam}}
\newcommand{\nestb}{{\sf pragam-b}}
\newcommand{\mcn}{{\sf M$^3$N}}
\newcommand{\expgrad}{{\sf ExpGrad}}
\newcommand{\smo}{{\sf SMO}}
\newcommand{\lasvm}{{\sf LaSVM}}
\newcommand{\sms}{{\sf SMS}}


\newcommand{\prbep}{{\sf PRBEP}}
\newcommand{\rocarea}{{\sf ROCArea}}
\newcommand{\pca}{\text{\sc pca}}

\newcommand{\arow}[2]{#1_{#2\cdot}}
\newcommand{\acol}[2]{#1_{\cdot#2}}
\newcommand{\expunder}[1]{\mathop{\EE}\limits_{#1}}
\newcommand{\mean}[1]{\mathop{\EE}\sbr{{#1}}}
%\newcommand{\vars}[2]{\var_{{#1}}\sbr{{#2}}}
\newcommand{\expec}[2]{\mathop{\EE}_{{#1}}\sbr{{#2}}}

\newcommand{\twoco}[1]{\multicolumn{2}{c|}{#1}}
\def\ci{\perp\!\!\!\perp}

\newcommand{\gstar}{g^{\star}}
\newcommand{\fstar}{f^{\star}}
\newcommand{\hstar}{h^{\star}}
\newcommand{\Astar}{A^{\star}}
\newcommand{\Kstar}{K^{\star}}

%\newcommand{\var}{\mathrm{Var}}
\newcommand{\grad}{{\nabla}}
\newcommand{\gradtil}{{\tilde{\grad}}}
\newcommand{\MED}{{\text{MED}}}
\newcommand{\where}{{\quad \text{where} \quad}}
\newcommand{\lcg}{{\textit{l.c.g}}}
\newcommand{\cp}{\mathrm{cp}}
\newcommand{\err}{{\sf err}}

\newcommand{\ydiff}[2]{\delta(#1, #2)}
\newcommand{\ykdiff}[2]{\delta(#1, #2)^{\kappa}}
\newcommand{\myfdiff}[2]{\Delta f(#1, #2)}



==> relatedwork.tex <==
%!TEX root = aamas2015.tex

\section{Related work}

There has been a significant effort to empirically investigate $\lambda$,
typically using batch off-line computing and model-based techniques. 
%settings, with computationally intensive approaches that provide insights.
 Sutton and Singh \citet{sutton1994onstep} investigated tuning both $\alpha$ and $\lambda$. They proposed three algorithms, the first two assume the underlying MDP has no cycles, and the third makes use of an estimate of the transition probabilities and is thus of most interest in tabular domains. Singh and Dayan \citet{singh1996analytical} provided analytical expression for bias and variance, given the model.
They suggest that there is a largest feasible step-size $\alpha$, below which bias converges to zero and variance converges to a non-zero value, and above which bias and/or variance may diverge. 
%They further hypothesize that the largest feasible $\alpha$ increases for larger values of $\lambda$, and that larger feasible values of both lead to faster convergence.
Downey and Sanner \citet{downey2010temporal} used a Bayesian variant of TD learning, requiring a batch of samples and off-line computation, but did provide an empirical demonstration off optimally setting $\lambda$ after obtaining all the samples. Kearns and Singh\citet{kearns2000bias} compute a bias-variance error bound for a modification of TD called phased TD. In each discrete phase the algorithm is given $n$ trajectories from each state. Because we have $n$ trajectories in each state the effective learning rate is $1/n$ removing the complexities of sample averaging in the conventional online TD-update. 
 %This modified algorithm makes the analysis easier which appears to be a common trend in the literature on this and related topics. 
 The error bounds are useful for, among other things, computing a new $\lambda$ value for each phase which outperforms any fixed $\lambda$ value, empirically demonstrating the utility of changing $\lambda$. 

There has also been a significant effort to theoretically characterizing $\lambda$.
%Aside from these three studies of directly trying to adjust $\lambda$, the remainder of related work involves the analysis of incremental, approximation value estimation algorithms. 
Most notably, the work of Schapire and Warmuth \cite{schapire1996ontheworst} contributed a finite sample analysis of incremental TD-style algorithms. They analyze a variant of TD called TD$^\star(\lambda)$, which although still linear and incremental,
computes value estimates quite differently. 
%They just of their bound was to characterized the squared loss of the predictions made by TD$^\star(\lambda)$ compared to the true values, after $t$ steps, in terms of (1) the loss of the best linear weight vector, (2) 2-norm difference between the initial weight vector and the vector corresponding to the best linear predictor, and (3) the step size, discount factor, and a constant bounding the norm of the eligibility trace. 
The resulting finite sample bound is particularly interesting, as it does not rely on model assumptions,
%but rather poses the result 
using only access to 
%The really nice thing about this bound is, it a finite sample bound, and it makes no assumptions about rewards, states, or transition functions, that is no reliance on the MDP framework; just 
a sequence of feature vectors, rewards and returns. 
Unfortunately, the bound cannot be analytically minimized to produce an optimal $\lambda$ value. 
They did simulate their bound, further verifying the intuition that
$\lambda$ should be larger if the best linear predictor is inaccurate, small if accurate and an intermediate value
otherwise. 
%and found that $\lambda$ between 0 and 1 were best depending on the magnitude of the loss incurred by the best linear predictor: (1) if the best you can do is high error (loss of best linear predictor is high), then $\lambda$ near 1.0 is best, (2) if the best you can do is low error, then the best $\lambda$ was near zero, and (3) intermediate $\lambda$ for intermediate losses.
%It is not clear how Schapire and Warmuth ended up with the TD$^\star(\lambda)$. They say its a true gradient descent algorithm for the L2 loss between the prediction and return, but provided no derivation. It appears they tried to compute there bounds for conventional TD$(\lambda)$, couldn't, and then worked backwards to figure out the modification to the algorithm that could complete their analysis. It is not clear from the proof, but later work suggests the key bit is being a true gradient algorithm. 
Li \citet{li2008aworst} later derived similar bounds for another gradient descent algorithm, called residual gradient. This algorithm, however, does not utilize eligibility traces and converges to a different solution than TD methods when function approximation is used \cite{sutton2009fast}. 
%\citet{kearns2000bias} also attempt to characterize $\lambda$ with their bias-variance analysis. 

Another approach involves removing the $\lambda$ parameter altogether, in an effort to improve robustness.
Konidaris et al. \citet{konidaris2011td} introduced a new TD method called TD$_\gamma$.
%though an incremental form of their algorithm introduces a similar meta-parameter (called $C$).
Their work defines a plausible set of assumptions implicitly made when constructing the $\lambda$-returns, and then relaxes one
of those assumptions. They derive an exact (but computationally expensive) algorithm, TD$_\gamma$, that no longer depends on a choice of $\lambda$
and performs well empirically in a variety of policy learning benchmarks. The incremental approximation to TD$_\gamma$ also performs reasonably well, but appears to be somewhat sensitive to the choice of
meta parameter $C$, and often requires large $C$ values to obtain good performance. This can be problematic,
as the complexity grows as $O(C \xdim)$, where $\xdim$ is the length of the trajectories---not linearly in the feature vector size. Nonetheless, TD$_\gamma$ constitutes a reasonable way to reduce parameter sensitivity in the on-policy setting.
%A different strategy has been to replace the $\lambda$ parameter all-together \cite{konidaris2011td}. The idea there is to
%take some of the assumptions behind $n$-step returns that define $\lambda$-returns, and relax them. The resulting
%algorithm no longer relies on a $\lambda$ parameter. We will compare to this algorithm,
%which is currently one of the only algorithms that enables a $\lambda$-like selecting criteria incrementally. 
Garcia and Serre\citet{garcia2001from} proposed a variant of Q-learning, for which the optimal value of $\lambda$ can be computed online. Their analysis, however, was restricted to the tabular case.
Finally, Mahmood et al. \citet{mahmood2014weighted} introduced weighted importance sampling
for off-policy learning; though indirect,
this is a strategy for enabling larger $\lambda$ to be selected, without destabilizing off-policy learning. 

This related work has helped shape our intuition on the role of $\lambda$,
and, in special cases, provided effective strategies for adapting $\lambda$.
%Particular experimental studies have also suggested reasonable
%heuristics. 
%Meta-parameter optimization is a critical topic for reinforcement learning, and each work constitutes a concrete step towards parameter-free (or parameter-reduced) reinforcement learning. 
In the next section, we add to existing work with
an empirical demonstration of \lamname, the first $\lambda$-adaptation algorithm
for off-policy, incremental learning,
developed from a well-defined, greedy objective. 
 
%There has been little work on finding an algorithm for setting $\lambda$. 

%Mannor et al (2004) investigated computing the bias and variance of value function estimation, but restricted the focus to the tabular cause and model-based algorithms that estimate the R and and transition functions and thus $\lambda$ plays no role.

%DAVID SILVERS COMMENT:
%The parameter ? is believed to trade off bias and variance [15]. \cite{singh1996analytical} explicitly examine the relationship between the bias and variance of value function estimates. They analyse the performance of offline TD(?) in terms of mean squared error. They compare MSE curves, using an offline analysis tool that requires a full model of the MDP, for a variety of constant values of ? and ?. They suggest that there is a largest feasible step-size ?, below which bias converges to zero and variance converges to a non-zero value, and above which bias and/or variance may diverge. They hypothesize that the largest feasible ? increases for larger values of ?, and furthermore that larger feasible values of ? and ? lead to faster convergence. They go

%Citations from RLDM:
%TODO: why did we cite kilter before?
%\cite{kolter2011thefixed}
%\cite{mahmood2014weighted}
%\cite{singh1996reinforcement}
%\cite{sutton1994onstep}
%\cite{szepesvari2010algorithms}
%\cite{sutton1998introduction}
%\cite{tesauro1992practical}
%\cite{vanseijen2014true}
%\cite{white2010interval}
%\cite{white2015thesis}


